Counting the dimension of splines of mixed smoothness: A general recipe, and its application to meshes of arbitrary topologies

In this paper we study the dimension of bivariate polynomial splines of mixed smoothness on polygonal meshes. Here, "mixed smoothness" refers to the choice of different orders of smoothness across different edges of the mesh. To study the dimension of spaces of such splines, we use tools from Homological Algebra. These tools were first applied to the study of splines by Billera (1988). Using them, estimation of the spline space dimension amounts to the study of the generalized Billera-Schenck-Stillman complex for the spline space. In particular, when the homology in positions one and zero of this complex are trivial, the dimension of the spline space can be computed combinatorially. We call such spline spaces "lower-acyclic." In this paper, starting from a spline space which is lower-acyclic, we present sufficient conditions that ensure that the same will be true for the spline space obtained after relaxing the smoothness requirements across a subset of the mesh edges. This general recipe is applied in a specific setting: meshes of arbitrary topologies. We show how our results can be used to compute the dimensions of spline spaces on triangulations, polygonal meshes, and T-meshes with holes.

==> setup/commands_simp.tex <==
%%%%%% NEW COMMANDS %%%%%%%%


\newcommand{\degreeDiff}{d^\face}

\newcommand{\minDegreeu}{{\check{\degreeu}}}
\newcommand{\minDegreev}{{\check{\degreev}}}
\newcommand{\maxDegreeu}{{\bar{\degreeu}}}
\newcommand{\maxDegreev}{{\bar{\degreev}}}
\newcommand{\polyTotal}[1]{\mathbb{P}_{#1}}
\newcommand{\polyRing}{R}
\newcommand{\polyRingH}{S}
\newcommand{\ideal}{\mathfrak{J}}
\newcommand{\idealL}{\mathfrak{L}}
\newcommand{\shiftideal}[3]{\mathfrak{#1}_{#2}(#3)}


\newcommand{\krond}[2]{\varepsilon_{#1, #2}}
\newcommand{\kronFE}[2]{\krond{\face_{#1}}{\edge_{#2}}}
\newcommand{\kronEV}[2]{\krond{\edge_{#1}}{\vertex_{#2}}}


==> setup/commands_tmesh.tex <==

%%%%%% NEW COMMANDS %%%%%%%%

%% T-mesh
\newcommand{\ids}{\chi}
\newcommand{\ms}{\rho}
\newcommand{\sms}{\lambda}

%% Polynomials



\newcommand{\minDegree}{{\underline{\bdegree}}}
\newcommand{\maxDegree}{{\overline{\bdegree}}}





==> source_files/mike_changelog.tex <==
%I'm recording changes I've made to the files, and also making suggestions.

1.  I find the term geometry independent introduced in Definition~1.5 a bit misleading - to me this suggests that dimensions don't change if vertex positions are changed.  I imagine that what is meant by this is that only the local geometry around vertices matters.  One option would be to simply call these \textit{acyclic} (an acyclic chain complex is one whose homologies vanish).  (This is also a bit misleading since the top homology of Q^r doesn't vanish.)

2.  I think homogenization needs to be treated more carefully.  The vector spaces P_\sigma are defined without reference to an ambient polynomial ring -- the number of variables is not defined.  I'm guessing that the target audience may not be as familiar with the practice of homogenizing.

3.  When smoothness is reduced, `carving off' a face, the corresponding chain complexes may either include the `carved off' face or not include it.  The difference is superficial - either the corresponding term is left off or it is not, and it contributes an easily determined term to the dimension; it does not effect geometry independence.  However we should be careful to address this as it will probably lead to confusion.

Changes:  I made alot of edits starting with the couple of paragraphs just prior to equation (5), and ending with Corollary 3.10.  Basically this is on pages 7,8,9, and 10.  I was going to log them all, but it might be easier for you to just take a look!



==> tikz/myTikZCommands.tex <==
\definecolor{myBlue}{rgb} {0,0.4470,0.7410}
\definecolor{myRed}{rgb} {0.8500,0.3250,0.0980}
\definecolor{myGray1}{rgb} {0,0,0}
\definecolor{myGray2}{rgb} {0.6,0.6,0.6}
\definecolor{myGray3}{rgb} {0.45,0.45,0.45}
\definecolor{myGray4}{rgb} {0.8,0.8,0.8}
\definecolor{myGray5}{rgb} {0.55,0.55,0.55}

\definecolor{myCPlot1}{rgb} {0,    0.4470,    0.7410}
\definecolor{myCPlot2}{rgb} {0.8500,   0.3250,    0.0980}
\definecolor{myCPlot3}{rgb} {0.9290,    0.6940,    0.1250}
\definecolor{myCPlot4}{rgb} {0.4940,    0.1840,    0.5560}
\definecolor{myCPlot5}{rgb} {0.4660,    0.6740,    0.1880}
\definecolor{myCPlot6}{rgb} {0.3010,    0.7450,    0.9330}
\definecolor{myCPlot7}{rgb} {0.6350,    0.0780,    0.1840}

\definecolor{myCPColor}{rgb} {0.9255, 0.6941, 0.355}

\newcommand{\logLogSlope}[6]
{
	% #1. Relative offset in x direction.
	% #2. Width in x direction, so xA-xB.
	% #3. Relative offset in y direction.
	% #4. Slope d(y)/d(log10(x)).
	% #5. Plot options.
	
	\pgfplotsextra
	{
		\pgfkeysgetvalue{/pgfplots/xmin}{\xmin}
		\pgfkeysgetvalue{/pgfplots/xmax}{\xmax}
		\pgfkeysgetvalue{/pgfplots/ymin}{\ymin}
		\pgfkeysgetvalue{/pgfplots/ymax}{\ymax}
		
		% Calculate auxilliary quantities, in relative sense.
		\pgfmathsetmacro{\xArel}{#1}
		\pgfmathsetmacro{\yArel}{#3}
		\pgfmathsetmacro{\xBrel}{#1-#2}
		\pgfmathsetmacro{\yBrel}{\yArel}
		\pgfmathsetmacro{\xCrel}{\xArel}
		%\pgfmathsetmacro{\yCrel}{ln(\yC/exp(\ymin))/ln(exp(\ymax)/exp(\ymin))} % REPLACE THIS EXPRESSION WITH AN EXPRESSION INDEPENDENT OF \yC TO PREVENT THE 'DIMENSION TOO LARGE' ERROR.
		
		\pgfmathsetmacro{\lnxB}{\xmin*(1-(#1-#2))+\xmax*(#1-#2)} % in [xmin,xmax].
		\pgfmathsetmacro{\lnxA}{\xmin*(1-#1)+\xmax*#1} % in [xmin,xmax].
		\pgfmathsetmacro{\lnyA}{\ymin*(1-#3)+\ymax*#3} % in [ymin,ymax].
		\pgfmathsetmacro{\lnyC}{\lnyA+#4*(\lnxA-\lnxB)}
		\pgfmathsetmacro{\yCrel}{\lnyC-\ymin)/(\ymax-\ymin)}
		
		% Define coordinates for \draw. MIND THE 'rel axis cs' as opposed to the 'axis cs'.
		\coordinate (A) at (rel axis cs:\xArel,\yArel);
		\coordinate (B) at (rel axis cs:\xBrel,\yBrel);
		\coordinate (C) at (rel axis cs:\xCrel,\yCrel);
		
		% Draw slope triangle.
		\draw[#5]   (B) -- (C) node[midway,#6] {#4};
	}
}

\tikzstyle{scpColor}=[circle, fill=myCPColor]

\tikzset{
	show curve controls/.style={
		decoration={
			show path construction,
			curveto code={
				\draw[myGray1,dashed,eThickness]
				(\tikzinputsegmentfirst)
				-- (\tikzinputsegmentsupporta)
				-- (\tikzinputsegmentsupportb)
				-- (\tikzinputsegmentlast)
				;
				\fill[scpColor] (\tikzinputsegmentfirst) circle(3pt);
				\fill[scpColor] (\tikzinputsegmentsupporta) circle(3pt);
				\fill[scpColor] (\tikzinputsegmentsupportb) circle(3pt);
				\fill[scpColor] (\tikzinputsegmentlast) circle(3pt);
				\draw[#1,line width=1pt]
				(\tikzinputsegmentfirst)
				.. controls (\tikzinputsegmentsupporta)
				and (\tikzinputsegmentsupportb) ..
				(\tikzinputsegmentlast);
			}
		},decorate
	}
}

\tikzset{
	% style to apply some styles to each segment of a path
	on each segment/.style={
		decorate,
		decoration={
			show path construction,
			moveto code={},
			lineto code={
				\path [#1]
				(\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
			},
			curveto code={
				\path [#1] (\tikzinputsegmentfirst)
				.. controls
				(\tikzinputsegmentsupporta) and (\tikzinputsegmentsupportb)
				..
				(\tikzinputsegmentlast);
			},
			closepath code={
				\path [#1]
				(\tikzinputsegmentfirst) -- (\tikzinputsegmentlast);
			},
		},
	},
	% style to add an arrow in the middle of a path
	mid arrow/.style={postaction={decorate,decoration={
				markings,
				mark=at position .6 with {\arrow[#1]{Latex}}
	}}},
}

\tikzset{
	bThickness/.style={line width=#1\pgflinewidth},
	bThickness/.default={2},
}

\tikzset{
	eThickness/.style={line width=#1\pgflinewidth},
	eThickness/.default={0.5},
}

\tikzset{cross/.style={cross out, draw, 
		minimum size=2*(#1-\pgflinewidth), 
		inner sep=0pt, outer sep=0pt}}

\pgfooclass{bezier quad}{
	
	\attribute vertex 0;
	\attribute vertex 1;
	\attribute vertex 2;
	\attribute vertex 3;
	\attribute degree 0;
	\attribute degree 1;
	
	\method bezier quad(){
		% the constructor; does nothing
	}
	
	\method set vertices(#1,#2,#3,#4,#5,#6,#7,#8) {
		% set the corners of the element
		\pgfcoordinate{vertex 0}{\pgfpoint{#1}{#2}}
		\pgfcoordinate{vertex 1}{\pgfpoint{#3}{#4}}
		\pgfcoordinate{vertex 2}{\pgfpoint{#5}{#6}}
		\pgfcoordinate{vertex 3}{\pgfpoint{#7}{#8}}
	}
	
	\method set rectangle vertices(#1,#2,#3,#4) {
		% set the corners of a rectangular element
		\pgfmathsetmacro{\xz}{#1}
		\pgfmathsetmacro{\yz}{#2}
		\pgfmathsetmacro{\xo}{#1+#3}
		\pgfmathsetmacro{\yo}{#2+#4}
		\pgfoothis.set vertices(\xz,\yz,\xo,\yz,\xo,\yo,\xz,\yo);
	}
	
	\method set vertex nodes(#1,#2,#3,#4) {
		% set the corners of the element
		\pgfcoordinate{vertex 0}{\pgfpointanchor{#1}{center}}
		\pgfcoordinate{vertex 1}{\pgfpointanchor{#2}{center}}
		\pgfcoordinate{vertex 2}{\pgfpointanchor{#3}{center}}
		\pgfcoordinate{vertex 3}{\pgfpointanchor{#4}{center}}
	}
	
	\method set degrees(#1,#2) {
		% set the polynomial degree
		\pgfooset{degree 0}{#1}
		\pgfooset{degree 1}{#2}
	}
	
	\method plot boundary() {
		% plot element boundary
		\draw[eThickness, black] (vertex 0) -- (vertex 1) -- (vertex 2) -- (vertex 3) -- cycle;
	}

	\method plot domain point(#1,#2,#3,#4,#5,#6,#7) {
		\node [draw, black, fill=#7, shape=circle, minimum size=3pt, anchor=center,scale=#1] (domain point #6) at (barycentric cs:b0=#2,b1=#3,b2=#4,b3=#5) {};
	}

	\method set domain extent() {
		% plot domain points for the element
		\coordinate (b0) at (barycentric cs:vertex 0=1,vertex 1=0.05,vertex 2=0.05,vertex 3=0.05) {};
		\coordinate (b1) at (barycentric cs:vertex 0=0.05,vertex 1=1,vertex 2=0.05,vertex 3=0.05) {};
		\coordinate (b2) at (barycentric cs:vertex 0=0.05,vertex 1=0.05,vertex 2=1,vertex 3=0.05) {};
		\coordinate (b3) at (barycentric cs:vertex 0=0.05,vertex 1=0.05,vertex 2=0.05,vertex 3=1) {};
	}
	
	\method plot domain points(#1,#2) {
		% plot domain points for the element
		\pgfmathtruncatemacro{\pzero}{\pgfoovalueof{degree 0}}
		\pgfmathtruncatemacro{\pone}{\pgfoovalueof{degree 1}}
		\pgfoothis.mark domain pts(0,\pzero,0,\pone,#1,#2)
	}
	
	\method plot extended boundary() {
		% plot element boundary and extend with dashed lines near corners
		\draw[eThickness, black] (vertex 0) -- (vertex 1) -- (vertex 2) -- (vertex 3) -- cycle;
		\foreach \x/\y in {0/1,1/2,2/3,3/0}{
			\draw[eThickness, dashed, black] (vertex \x) -- ($(vertex \y)!1.1!(vertex \x)$);
			\draw[eThickness, dashed, black] (vertex \y) -- ($(vertex \x)!1.1!(vertex \y)$);
		}
	}
	
	\method label vertices(#1,#2,#3,#4,#5) {
		% label corner vertices
		\node [scale=#5] at (vertex 0) {#1};
		\node [scale=#5] at (vertex 1) {#2};
		\node [scale=#5] at (vertex 2) {#3};
		\node [scale=#5] at (vertex 3) {#4};
	}
	
	\method label edges(#1,#2,#3,#4,#5) {
		% label boundary edges
		\node [scale=#5] at ($(vertex 0)!0.5!(vertex 1)$) {#1};
		\node [scale=#5] at ($(vertex 1)!0.5!(vertex 2)$) {#2};
		\node [scale=#5] at ($(vertex 2)!0.5!(vertex 3)$) {#3};
		\node [scale=#5] at ($(vertex 3)!0.5!(vertex 0)$) {#4};
	}
	
	\method label face(#1,#2) {
		% label face
		\node [anchor=center,scale=#2] at (barycentric cs:vertex 0=0.25,vertex 1=0.25,vertex 2=0.25,vertex 3=0.25) {#1};
	}

	\method shade face(#1) {
		% label face
		\draw[eThickness, black, fill=#1] (vertex 0) -- (vertex 1) -- (vertex 2) -- (vertex 3) -- cycle;
	}

	\method mark domain pts(#1,#2,#3,#4,#5,#6) {
		% mark points
		\pgfoothis.set domain extent();
		\pgfmathtruncatemacro{\pzero}{\pgfoovalueof{degree 0}}
		\pgfmathtruncatemacro{\pone}{\pgfoovalueof{degree 1}}
		\foreach \i in {#1,...,#2}{
			\foreach \j in {#3,...,#4}{
				\pgfmathsetmacro{\a}{\i/\pzero}
				\pgfmathsetmacro{\b}{\j/\pone}
				\pgfmathsetmacro{\aone}{(1-\a)*(1-\b)}
				\pgfmathsetmacro{\atwo}{(\a)*(1-\b)}
				\pgfmathsetmacro{\athree}{(\a)*(\b)}
				\pgfmathsetmacro{\afour}{(1-\a)*(\b)}
				\pgfoothis.plot domain point(#5,\aone,\atwo,\athree,\afour,\i\j, #6)
			}
		}
	}

	\method mark edge pts(#1,#2,#3,#4) {
		% mark points
		{
			\ifthenelse{#1 = 0}{
				\pgfmathtruncatemacro{\iz}{0}
				\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
				\pgfmathtruncatemacro{\jz}{0}
				\pgfmathtruncatemacro{\jo}{#2}
				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#3,#4)
			}{};}
	
		{\ifthenelse{#1=1}{
			\pgfmathtruncatemacro{\iz}{\pgfoovalueof{degree 0} - #2}
			\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
			\pgfmathtruncatemacro{\jz}{0}
			\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
			\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#3,#4)
		}{};}

		{\ifthenelse{#1=2}{
			\pgfmathtruncatemacro{\iz}{0}
			\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
			\pgfmathtruncatemacro{\jz}{\pgfoovalueof{degree 1}-#2}
			\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
			\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#3,#4)
		}{};}

		{\ifthenelse{#1=3}{
			\pgfmathtruncatemacro{\iz}{0}
			\pgfmathtruncatemacro{\io}{#2}
			\pgfmathtruncatemacro{\jz}{0}
			\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
			\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#3,#4)
		}{};}
	}

	\method mark vertex pts(#1,#2,#3,#4,#5) {
		% mark points
		{
			\ifthenelse{#1 = 0}{
				\pgfmathtruncatemacro{\iz}{0}
				\pgfmathtruncatemacro{\io}{#2}
				\pgfmathtruncatemacro{\jz}{0}
				\pgfmathtruncatemacro{\jo}{#3}
				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#4,#5)
			}{};}
		
		{\ifthenelse{#1=1}{
				\pgfmathtruncatemacro{\iz}{\pgfoovalueof{degree 0} - #2}
				\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
				\pgfmathtruncatemacro{\jz}{0}
				\pgfmathtruncatemacro{\jo}{#3}
				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#4,#5)
			}{};}
		
		{\ifthenelse{#1=2}{
				\pgfmathtruncatemacro{\iz}{\pgfoovalueof{degree 0} - #2}
				\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
				\pgfmathtruncatemacro{\jz}{\pgfoovalueof{degree 1}-#3}
				\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#4,#5)
			}{};}
		
		{\ifthenelse{#1=3}{
				\pgfmathtruncatemacro{\iz}{0}
				\pgfmathtruncatemacro{\io}{#2}
				\pgfmathtruncatemacro{\jz}{\pgfoovalueof{degree 1}-#3}
				\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#4,#5)
			}{};}
	}
}
\pgfoonew \bezier=new bezier quad()

%\pgfooclass{bezier edge}{
%	
%	\attribute vertex 0;
%	\attribute vertex 1;
%	\attribute degree 0;
%	
%	\method bezier edge(){
%		% the constructor; does nothing
%	}
%	
%	\method set vertices(#1,#2,#3,#4,#5,#6,#7,#8) {
%		% set the corners of the element
%		\pgfcoordinate{vertex 0}{\pgfpoint{#1}{#2}}
%		\pgfcoordinate{vertex 1}{\pgfpoint{#3}{#4}}
%		\pgfcoordinate{vertex 2}{\pgfpoint{#5}{#6}}
%		\pgfcoordinate{vertex 3}{\pgfpoint{#7}{#8}}
%	}
%	
%	\method set rectangle vertices(#1,#2,#3,#4) {
%		% set the corners of a rectangular element
%		\pgfmathsetmacro{\xz}{#1}
%		\pgfmathsetmacro{\yz}{#2}
%		\pgfmathsetmacro{\xo}{#1+#3}
%		\pgfmathsetmacro{\yo}{#2+#4}
%		\pgfoothis.set vertices(\xz,\yz,\xo,\yz,\xo,\yo,\xz,\yo);
%	}
%	
%	\method set vertex nodes(#1,#2,#3,#4) {
%		% set the corners of the element
%		\pgfcoordinate{vertex 0}{\pgfpointanchor{#1}{center}}
%		\pgfcoordinate{vertex 1}{\pgfpointanchor{#2}{center}}
%		\pgfcoordinate{vertex 2}{\pgfpointanchor{#3}{center}}
%		\pgfcoordinate{vertex 3}{\pgfpointanchor{#4}{center}}
%	}
%	
%	\method set degrees(#1,#2) {
%		% set the polynomial degree
%		\pgfooset{degree 0}{#1}
%		\pgfooset{degree 1}{#2}
%	}
%	
%	\method plot boundary() {
%		% plot element boundary
%		\draw[eThickness, black] (vertex 0) -- (vertex 1) -- (vertex 2) -- (vertex 3) -- cycle;
%	}
%	
%	\method plot domain point(#1,#2,#3,#4,#5,#6,#7) {
%		\node [draw, black, fill=#7, shape=circle, minimum size=3pt, anchor=center,scale=#1] (domain point #6) at (barycentric cs:b0=#2,b1=#3,b2=#4,b3=#5) {};
%	}
%	
%	\method set domain extent() {
%		% plot domain points for the element
%		\coordinate (b0) at (barycentric cs:vertex 0=1,vertex 1=0.05,vertex 2=0.05,vertex 3=0.05) {};
%		\coordinate (b1) at (barycentric cs:vertex 0=0.05,vertex 1=1,vertex 2=0.05,vertex 3=0.05) {};
%		\coordinate (b2) at (barycentric cs:vertex 0=0.05,vertex 1=0.05,vertex 2=1,vertex 3=0.05) {};
%		\coordinate (b3) at (barycentric cs:vertex 0=0.05,vertex 1=0.05,vertex 2=0.05,vertex 3=1) {};
%	}
%	
%	\method plot domain points(#1,#2) {
%		% plot domain points for the element
%		\pgfmathtruncatemacro{\pzero}{\pgfoovalueof{degree 0}}
%		\pgfmathtruncatemacro{\pone}{\pgfoovalueof{degree 1}}
%		\pgfoothis.mark domain pts(0,\pzero,0,\pone,#1,#2)
%	}
%	
%	\method plot extended boundary() {
%		% plot element boundary and extend with dashed lines near corners
%		\draw[eThickness, black] (vertex 0) -- (vertex 1) -- (vertex 2) -- (vertex 3) -- cycle;
%		\foreach \x/\y in {0/1,1/2,2/3,3/0}{
%			\draw[eThickness, dashed, black] (vertex \x) -- ($(vertex \y)!1.1!(vertex \x)$);
%			\draw[eThickness, dashed, black] (vertex \y) -- ($(vertex \x)!1.1!(vertex \y)$);
%		}
%	}
%	
%	\method label vertices(#1,#2,#3,#4,#5) {
%		% label corner vertices
%		\node [scale=#5] at (vertex 0) {#1};
%		\node [scale=#5] at (vertex 1) {#2};
%		\node [scale=#5] at (vertex 2) {#3};
%		\node [scale=#5] at (vertex 3) {#4};
%	}
%	
%	\method label edges(#1,#2,#3,#4,#5) {
%		% label boundary edges
%		\node [scale=#5] at ($(vertex 0)!0.5!(vertex 1)$) {#1};
%		\node [scale=#5] at ($(vertex 1)!0.5!(vertex 2)$) {#2};
%		\node [scale=#5] at ($(vertex 2)!0.5!(vertex 3)$) {#3};
%		\node [scale=#5] at ($(vertex 3)!0.5!(vertex 0)$) {#4};
%	}
%	
%	\method label face(#1,#2) {
%		% label face
%		\node [anchor=center,scale=#2] at (barycentric cs:vertex 0=0.25,vertex 1=0.25,vertex 2=0.25,vertex 3=0.25) {#1};
%	}
%	
%	\method mark domain pts(#1,#2,#3,#4,#5,#6) {
%		% mark points
%		\pgfoothis.set domain extent();
%		\pgfmathtruncatemacro{\pzero}{\pgfoovalueof{degree 0}}
%		\pgfmathtruncatemacro{\pone}{\pgfoovalueof{degree 1}}
%		\foreach \i in {#1,...,#2}{
%			\foreach \j in {#3,...,#4}{
%				\pgfmathsetmacro{\a}{\i/\pzero}
%				\pgfmathsetmacro{\b}{\j/\pone}
%				\pgfmathsetmacro{\aone}{(1-\a)*(1-\b)}
%				\pgfmathsetmacro{\atwo}{(\a)*(1-\b)}
%				\pgfmathsetmacro{\athree}{(\a)*(\b)}
%				\pgfmathsetmacro{\afour}{(1-\a)*(\b)}
%				\pgfoothis.plot domain point(#5,\aone,\atwo,\athree,\afour,\i\j, #6)
%			}
%		}
%	}
%	
%	\method mark edge pts(#1,#2,#3,#4) {
%		% mark points
%		{
%			\ifthenelse{#1 = 0}{
%				\pgfmathtruncatemacro{\iz}{0}
%				\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
%				\pgfmathtruncatemacro{\jz}{0}
%				\pgfmathtruncatemacro{\jo}{#2}
%				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#3,#4)
%			}{};}
%		
%		{\ifthenelse{#1=1}{
%				\pgfmathtruncatemacro{\iz}{\pgfoovalueof{degree 0} - #2}
%				\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
%				\pgfmathtruncatemacro{\jz}{0}
%				\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
%				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#3,#4)
%			}{};}
%		
%		{\ifthenelse{#1=2}{
%				\pgfmathtruncatemacro{\iz}{0}
%				\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
%				\pgfmathtruncatemacro{\jz}{\pgfoovalueof{degree 1}-#2}
%				\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
%				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#3,#4)
%			}{};}
%		
%		{\ifthenelse{#1=3}{
%				\pgfmathtruncatemacro{\iz}{0}
%				\pgfmathtruncatemacro{\io}{#2}
%				\pgfmathtruncatemacro{\jz}{0}
%				\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
%				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#3,#4)
%			}{};}
%	}
%	
%	\method mark vertex pts(#1,#2,#3,#4,#5) {
%		% mark points
%		{
%			\ifthenelse{#1 = 0}{
%				\pgfmathtruncatemacro{\iz}{0}
%				\pgfmathtruncatemacro{\io}{#2}
%				\pgfmathtruncatemacro{\jz}{0}
%				\pgfmathtruncatemacro{\jo}{#3}
%				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#4,#5)
%			}{};}
%		
%		{\ifthenelse{#1=1}{
%				\pgfmathtruncatemacro{\iz}{\pgfoovalueof{degree 0} - #2}
%				\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
%				\pgfmathtruncatemacro{\jz}{0}
%				\pgfmathtruncatemacro{\jo}{#3}
%				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#4,#5)
%			}{};}
%		
%		{\ifthenelse{#1=2}{
%				\pgfmathtruncatemacro{\iz}{\pgfoovalueof{degree 0} - #2}
%				\pgfmathtruncatemacro{\io}{\pgfoovalueof{degree 0}}
%				\pgfmathtruncatemacro{\jz}{\pgfoovalueof{degree 1}-#3}
%				\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
%				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#4,#5)
%			}{};}
%		
%		{\ifthenelse{#1=3}{
%				\pgfmathtruncatemacro{\iz}{0}
%				\pgfmathtruncatemacro{\io}{#2}
%				\pgfmathtruncatemacro{\jz}{\pgfoovalueof{degree 1}-#3}
%				\pgfmathtruncatemacro{\jo}{\pgfoovalueof{degree 1}}
%				\pgfoothis.mark domain pts(\iz,\io,\jz,\jo,#4,#5)
%			}{};}
%	}
%}
%\pgfoonew \bezier=new bezier edge()

%%% BEZIER ELEMENT
%\pgfooclass{myQuadElement}{ % This is the class stamp
%	\method myQuadElement() { % The constructor
%	}
%	\method plot(#1,#2,#3,#4,#5,#6,#7,#8) { % plot Bezier element
%		\begin{scope}
%			\draw[eThickness,black] (#1,#2) -- (#3,#4) -- (#5,#6) -- (#7,#8) -- cycle;
%			\node[coordinate] (v1) at (#1,#2) {};
%			\node[coordinate] (v2) at (#3,#4) {};
%			\node[coordinate] (v3) at (#5,#6) {};
%			\node[coordinate] (v4) at (#7,#8) {};
%		\end{scope}
%	}
%	\method plotColor(#1,#2,#3,#4,#5,#6,#7,#8,#9) { % plot Bezier element
%		\begin{scope}
%			\draw[eThickness,dashed,#9] (#1,#2) -- (#3,#4) -- (#5,#6) -- (#7,#8) -- cycle;
%			\node[coordinate] (v1) at (#1,#2) {};
%			\node[coordinate] (v2) at (#3,#4) {};
%			\node[coordinate] (v3) at (#5,#6) {};
%			\node[coordinate] (v4) at (#7,#8) {};
%		\end{scope}
%	}
%	\method plotInteriorDomainPoints(#1,#2,#3,#4,#5,#6) {
%		\begin{scope}
%			\pgfmathtruncatemacro{\p}{#5-1}
%			\foreach \x in {2,...,\p}{
%				\foreach \y in {2,...,\p}{
%					\pgfmathsetmacro{\a}{(\x-1)/(#5-1)}
%					\pgfmathsetmacro{\b}{(\y-1)/(#5-1)}
%					\pgfmathsetmacro{\aone}{(1-\a)*(1-\b)}
%					\pgfmathsetmacro{\atwo}{(\a)*(1-\b)}
%					\pgfmathsetmacro{\athree}{(\a)*(\b)}
%					\pgfmathsetmacro{\afour}{(1-\a)*(\b)}
%					\node [draw, black, shape=rectangle, minimum width=3pt, minimum height=3pt, anchor=center,scale=0.5,fill=#6] (b\x\y) at (barycentric cs:#1=\aone,#2=\atwo,#3=\athree,#4=\afour) {};
%				}
%			}
%		\end{scope}
%	}
%	\method plotEdgeDomainPoints(#1,#2,#3,#4,#5) {
%		\begin{scope}
%			\pgfmathtruncatemacro{\p}{#3-1}
%			\foreach \x in {2,...,\p}{
%				\pgfmathsetmacro{\a}{(\x-1)/(#3-1)}
%				\pgfmathsetmacro{\aone}{(1-\a)}
%				\pgfmathsetmacro{\atwo}{\a}
%				\node [draw, black, shape=rectangle, minimum width=3pt, minimum height=3pt, anchor=center,scale=0.5,fill=#5] (e#4\x) at (barycentric cs:#1=\aone,#2=\atwo) {};
%			}
%		\end{scope}
%	}
%	\method plotCorner(#1,#2,#3) {
%		\begin{scope}
%			\node [draw, black, shape=rectangle, minimum width=3pt, minimum height=3pt, anchor=center,scale=0.5,fill=#3] (c#2) at (#1) {};
%		\end{scope}
%	}
%}
%\pgfoonew \myQuad=new myQuadElement()
